LatentKeypointGAN: Controlling Images via Latent Keypoints -- Extended Abstract

Generative adversarial networks (GANs) can now generate photo-realistic images. However, how to best control the image content remains an open challenge. We introduce LatentKeypointGAN, a two-stage GAN internally conditioned on a set of keypoints and associated appearance embeddings providing control of the position and style of the generated objects and their respective parts. A major difficulty that we address is disentangling the image into spatial and appearance factors with little domain knowledge and supervision signals. We demonstrate in a user study and quantitative experiments that LatentKeypointGAN provides an interpretable latent space that can be used to re-arrange the generated images by re-positioning and exchanging keypoint embeddings, such as generating portraits by combining the eyes, and mouth from different images. Notably, our method does not require labels as it is self-supervised and thereby applies to diverse application domains, such as editing portraits, indoor rooms, and full-body human poses.

==> tex/related_works.tex <==
\section{Related Work} \label{sec:related_work}

In the following, we discuss variants of generative models that learn to synthesize images from a collection of examples, focusing on methods providing control on the image content. Table~\ref{tab:features} summarizes the editing features of the most-related methods.

\input{tex/tab_features}
%modeling keypoints and those 

\textbf{GANs}  \cite{goodfellow2014generative} are trained to generate images from a distribution that resembles the training distributions. Recent approaches attain photo-realism for portrait images. \cite{karras2018progressive} train a progressive growth of the GAN's generator and discriminator. After that, \cite{karras2019style, karras2020analyzing} integrate multiplicative neural network layers to build StyleGAN and StyleGAN2.
StyleGAN gains some control on the generated high-resolution, high-quality faces by 
adopting ideas from style transfer \cite{gatys2016image, huang2017arbitrary} and exchanging features of hidden layers between different samples. We build upon these network architectures and equip them with additional structure.


\textbf{Editing entire images with GANs.}
More recently, efforts have been made on exploring the latent space of a pre-trained StyleGAN for image editing \cite{shen2020interpreting, Jahanian*2020On}. To allow editing real-world images, various encoders \cite{zhu2020domain, abdal2019image2stylegan, abdal2020image2stylegan++, guan2020collaborative, wulff2020improving, richardson2020encoding} have been trained to project images into the latent space of StyleGANs. These methods provide control over the image synthesis process, such as for changing age, pose, gender, illumination and enable rig-like controls over semantic face parameters \cite{tewari2020stylerig, tewari2020pie, ghosh2020gif, deng2020disentangled} by conditioning on parametric face models \cite{blanz1999morphable, FLAME:SiggraphAsia2017}. 
Compared with these methods, our model focuses on detailed and local semantic controls. Instead of changing the face as a whole, our method is able to change a local patch without an unwanted impact on other regions. Furthermore, our keypoints provide control handles for animation without manual rigging, making it easily applicable to different objects and image domains. 

\textbf{Editing images locally with unconditional GANs.} Instead of exchanging entire feature maps for style editing, local modifications are possible but require care to maintain consistent and artifact-free synthesis. \cite{collins2020editing} propose to cluster regions in the feature maps of StyleGAN that have similar activation and to edit images by exchanging clusters. But this requires human supervision to select suitable clusters and can lead to artifacts since the network was not trained on this editing task. In a similar vein, \cite{kwon2021diagonal} manipulate attention maps to edit the pose and local shape, but they do not demonstrate local appearance editing.
Instead of using existing feature maps, \cite{alharbi2020disentangled} and \cite{kim2021exploiting} train spatially-variable maps by 
structured noise generators, which improves feature editing at inference. However, this requires to 'paint' source and target feature regions by hand for every instance. By contrast, our model provides a higher-level control to \textit{explicitly} change the pose by modifying keypoint locations that are consistent across images. While enabling very useful forms of editing, all of the methods above require some form of a pixel-level selection of regions at test time or manual cluster selection out of hundreds of candidates after training.
As a result, they provide limited spatial editing control. Neither of them demonstrates moving parts relative to each other or adding and removing parts. Most existing methods that achieve part addition and removal either use available segmentation masks \cite{poisson2003,rav2008unwrap,lu2020, kasten2021layered,lu2021omnimatte} or require separate datasets with and without that part (e.g., faces with and without glasses) \cite{zhan2019spatial,tsai2017deep}.  More recent works \cite{BlockGAN2020, niemeyer2021giraffe} learn to rotate, add, or move entire objects in an unsupervised manner, but their setting does not work on modeling parts.
In sum, our keypoint-based editing is both more intuitive and enables additional editing capabilities.
%Besides, our keypoint based editing is more intuitive and more explicit editing than the feature map based methods.

\textbf{Mask-conditional image synthesis} methods synthesize images that resemble a given reference segmentation mask \cite{sola2017image,zhu2017unpaired,park2019semantic}.
\cite{park2019semantic} pioneered using spatially-adaptive denormalization (SPADE) to transfer segmentation masks to images, which we borrow and adapt to be conditioned on landmark position. To control individual aspects of faces, such as changing eye or nose shape, recent works \cite{zhu2020sean, tan2021efficient, tan2021diverse}
% tan2020michigan
further modify SPADE to allow local editing on images. Compared with these methods, our model does not take any kind of supervision or other conditions at training time. It is trained in a totally unsupervised manner and therefore eases the application to new domains for which no labels exist. Still, our method allows the landmarks to learn a meaningful location and semantic embedding that can be controlled at test time. 
%\HR{This section is a long list, we probably only want to retain the most recent ones and those in SIGGRAPH (no matter which time)}

% \textbf{Conditional image synthesis} methods synthesize images that resemble a given reference input, such as category labels \cite{mirza2014conditional, odena2017conditional}, text \cite{zhang2017stackgan, reed2016generative}, and layout \cite{zhao2019image, sun2019image}. A variant of the conditional GANs can do image-to-image translation \cite{isola2017image, huang2018multimodal, liu2017unsupervised, zhu2017toward, zhu2017unpaired, wang2018high, park2019semantic}. These approaches aim to transfer images from one domain to another while preserving the image structure, such as mapping from day to night. \cite{park2019semantic} pioneered using spatially-adaptive normalization to transfer segmentation masks to images, which we borrow and adapt to be conditioned on landmark position. To control individual aspects of faces, such as changing eye or nose shape, recent works condition on segmentation masks \cite{lee2020maskgan, yu2020toward, richardson2020encoding, zhu2020sean, tan2020semantic}, rough sketches \cite{tseng2020artediting, chen2020deepfacedrawing}, landmarks \cite{yang2019exposing}, or word labels such as with or w/o glasses  \cite{cheng2020segvae},  of faces as input. \cite{hong2018learning} can superimpose a new object without requiring an exact mask but still require one at training time. Compared with these methods, our model does not take any kind of supervision or other conditions at training time. It is trained in a totally unsupervised manner and therefore eases the application to new domains for which no labels exist. Still, our method allows the landmarks to learn a meaningful location and semantic embedding that can be controlled at test time. \HR{This section is a long list, we probably only want to retain the most recent ones and those in SIGGRAPH (no matter which time)}

% \textbf{Unsupervised landmark discovery} approaches aim to detect the landmarks from images without supervision. Most works train two-branch autoencoders, where shape and appearance are disentangled by training on pairs of images where one of the two is matching while the other factor varies. The essence of these methods is to compare the pair of images to discover disentangled landmarks. These pairs can stem from different views \cite{suwajanakorn2018discovery, Rhodin_2019_CVPR}, and frames of the same video \cite{siarohin2019animating, kulkarni2019unsupervised, minderer2019unsupervised}. However, this additional motion information is not always available or is difficult to capture. Existing unsupervised methods trained on single images create pairs from spatial deformation and color shifts of a source image \cite{xing2018deformable, shu2018deforming, thewlis2019unsupervised, li2020unsupervised, cheng2020unsupervised, dundar2020unsupervised}. Yet, the parameters of augmentation strategies, such as the commonly used thin-plate spline deformation model \cite{thewlis2017unsupervised, zhang2018unsupervised, jakab2018unsupervised, lorenz2019unsupervised}, are difficult to calibrate and image quality is lower than for GANs.
% %and the learned keypoints may be biased to be only meaningful for the transformation \cite{li2020unsupervised}. 
% %Besides, the appearance information may be hidden in keypoint location \cite{xu2020unsupervised}. 
% Moreover, the cycle consistency-based methods \cite{wu2019transgaga, xu2020unsupervised} cannot provide local editing ability. 
% By contrast, We show that our generator can all-together disentangle the appearance and keypoint location, control the images locally, and provides an improved image quality. 
% %Furthermore, the underlying idea of these methods, no matter whether they depend on multi-views, videos, or thin-plate splines, is creating pairs of images to compare to find the clue of equivariant keypoints in comparison. On the other hand, our method does not need any paired correspondences. It is totally based on generation. 
% %Our GAN approach poses a viable alternative by training a keypoint detector on synthetic examples generated by LatentKeypointGAN. 
% \HR{We may want to remove or shorten this paragraph significantly} \xz{How about removing it? I think SIGGRAPH does not care too much at this part?}\HR{If so, we should make sure that we cite the most important works in the intro (where we discuss the autoencoder work} \xz{I have cited the most important works in the intro. Just wondering if we could move this part to appendix?}
